Enhancements of Discretization Approaches for Non-Convex Mixed-Integer Quadratically Constraint Quadratic Programming: Part I

We study mixed-integer programming (MIP) relaxation techniques for the solution of non convex mixed-integer quadratically constrained quadratic programs (MIQCQPs). We present MIP relaxation methods for non convex continuous variable products. In Part I, we consider MIP relaxations based on separable reformulation. The main focus is the introduction of the enhanced separable MIP relaxation for nonconvex quadratic products of the form z=xy, called hybrid separable (HybS). Additionally, we introduce a logarithmic MIP relaxation for univariate quadratic terms, called sawtooth relaxation. We combine the latter with HybS and existing separable reformulations to derive MIP relaxations of MIQCQPs. We provide a comprehensive theoretical analysis of these techniques, underlining the theoretical advantages of HybS compared to its predecessors. We perform a broad computational study to demonstrate the effectiveness of the enhanced MIP relaxation in terms of producing tight dual bounds for MIQCQPs. In Part II, we study MIP relaxations that extend the well-known MIP relaxation normalized multiparametric disaggregation technique (NMDT) and present further theoretical and computational analyses.

==> latexmkrc <==
use File::Basename;
use File::Copy;
use File::Spec::Functions 'file_name_is_absolute';
use Cwd 'abs_path';
use File::Path 'make_path';

sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        $base_name =~ s/\.tex$//;  # Remove .tex extension
        pushd $path;

        # Only compile if .aux file does not exist
        unless (-e "$base_name.aux") {
            my $return = system "latexmk",
                                @sub_doc_options,
                                "-aux-directory=$sub_doc_output",
                                "-output-directory=$sub_doc_output",
                                $base_name;

            if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
                 # Make sure the output directory exists before trying to write to it
                 unless (-e $sub_doc_output or mkdir $sub_doc_output) {
                     die "Unable to create directory $sub_doc_output\n";
                 }

                 rdb_add_generated( "$sub_doc_output/$base_name.aux" );
                 copy "$sub_doc_output/$base_name.aux", ".";
            }
            popd;
            return $return;
        }
   }
}

